JanusDNA: A Powerful Bi-directional Hybrid DNA Foundation Model

Large language models (LLMs) have revolutionized natural language processing and are increasingly applied to other sequential data types, including genetic sequences. However, adapting LLMs to genomics presents significant challenges. Capturing complex genomic interactions requires modeling long-range dependencies within DNA sequences, where interactions often span over 10,000 base pairs, even within a single gene, posing substantial computational burdens under conventional model architectures and training paradigms. Moreover, standard LLM training approaches are suboptimal for DNA: autoregressive training, while efficient, supports only unidirectional understanding. However, DNA is inherently bidirectional, e.g., bidirectional promoters regulate transcription in both directions and account for nearly 11% of human gene expression. Masked language models (MLMs) allow bidirectional understanding but are inefficient, as only masked tokens contribute to the loss per step. To address these limitations, we introduce JanusDNA, the first bidirectional DNA foundation model built upon a novel pretraining paradigm that combines the optimization efficiency of autoregressive modeling with the bidirectional comprehension of masked modeling. JanusDNA adopts a hybrid Mamba, Attention and Mixture of Experts (MoE) architecture, combining long-range modeling of Attention with efficient sequential learning of Mamba. MoE layers further scale model capacity via sparse activation while keeping computational cost low. Notably, JanusDNA processes up to 1 million base pairs at single nucleotide resolution on a single 80GB GPU. Extensive experiments and ablations show JanusDNA achieves new SOTA results on three genomic representation benchmarks, outperforming models with 250x more activated parameters. Code: https://github.com/Qihao-Duan/JanusDNA

==> tables/ablation_clm_mlm_.tex <==
\begin{table}[t]
    \centering
    \caption{Results for Last Token.}
    \label{tab:last_token}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{janus} & \multicolumn{3}{c}{clm} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    size(M) & 0.056 & 0.207 & 0.795 & 0.061 & 0.209 & 0.814 \\
    step(k)$\backslash$dim & 32 & 64 & 128 & 40 & 76 & 152 \\
    \midrule
    1 & 0.428 & 0.439 & 0.445 & 0.421 & 0.426 & 0.434 \\
    2 & 0.445 & 0.451 & 0.460 & 0.454 & 0.441 & 0.453 \\
    3 & 0.450 & 0.462 & 0.472 & 0.443 & 0.447 & 0.471 \\
    4 & 0.451 & 0.466 & 0.473 & 0.443 & 0.451 & 0.468 \\
    5 & 0.453 & 0.470 & 0.479 & 0.454 & 0.457 & 0.478 \\
    6 & 0.455 & 0.473 & 0.482 & 0.451 & 0.453 & 0.481 \\
    7 & 0.458 & 0.474 & 0.484 & 0.449 & 0.457 & 0.482 \\
    8 & 0.459 & 0.477 & 0.488 & 0.459 & 0.465 & 0.479 \\
    9 & 0.461 & 0.479 & 0.490 & 0.453 & 0.467 & 0.479 \\
    10 & 0.461 & 0.480 & 0.491 & 0.459 & 0.465 & 0.484 \\
    \bottomrule
    \end{tabular}
    \end{table}
    
    \begin{table}[t]
    \centering
    \caption{Results for Middle Token.}
    \label{tab:middle_token}
    \small
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{janus} & \multicolumn{3}{c}{clm} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    size(M) & 0.056 & 0.207 & 0.795 & 0.061 & 0.209 & 0.814 \\
    step(k)$\backslash$dim & 32 & 64 & 128 & 40 & 76 & 152 \\
    \midrule
    1 & 0.428 & 0.436 & 0.440 & 0.384 & 0.400 & 0.408 \\
    2 & 0.438 & 0.454 & 0.465 & 0.429 & 0.425 & 0.443 \\
    3 & 0.437 & 0.449 & 0.467 & 0.436 & 0.446 & 0.454 \\
    4 & 0.443 & 0.465 & 0.471 & 0.434 & 0.451 & 0.454 \\
    5 & 0.444 & 0.477 & 0.477 & 0.434 & 0.449 & 0.451 \\
    6 & 0.456 & 0.474 & 0.482 & 0.428 & 0.442 & 0.446 \\
    7 & 0.458 & 0.471 & 0.477 & 0.438 & 0.457 & 0.461 \\
    8 & 0.453 & 0.478 & 0.478 & 0.434 & 0.455 & 0.461 \\
    9 & 0.458 & 0.481 & 0.485 & 0.447 & 0.458 & 0.465 \\
    10 & 0.456 & 0.482 & 0.488 & 0.443 & 0.456 & 0.465 \\
    \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{table}

==> tables/gb_ablation_dimscale.tex <==
\begin{table*}[h!]
\centering
\caption{Performance comparison of models on genomic benchmarks. Accuracy values with error bars (\tiny{\pm) are reported.}
\label{tab:model_comparison}
\begin{scriptsize}
\begin{sc}
\begin{tabular}{l@{\hskip 0.2em}c@{\hskip 0.2em}c@{\hskip 0.2em}c@{\hskip 0.2em}c@{\hskip 0.2em}c@{\hskip 0.2em}c}
\toprule
\textbf{Dataset} & \textbf{OnlyMoE-32} & \textbf{OnlyMoE-72} & \textbf{OnlyMoE-128} & \textbf{Attn-32} & \textbf{Attn-72} & \textbf{Attn-128} \\ 
\midrule
Human OCR Ensembl       & $0.825$\tiny{$\pm0.002$} & $0.829$\tiny{$\pm0.002$} & $0.832$\tiny{$\pm0.005$} & $0.826$\tiny{$\pm0.002$} & $0.828$\tiny{$\pm0.003$} & $0.833$\tiny{$\pm0.002$} \\
Human NonTATA Promoters & $0.940$\tiny{$\pm0.004$} & $0.962$\tiny{$\pm0.003$} & $0.938$\tiny{$\pm0.025$} & $0.940$\tiny{$\pm0.005$} & $0.964$\tiny{$\pm0.008$} & $0.965$\tiny{$\pm0.007$} \\
Human Regulatory        & $0.862$\tiny{$\pm0.009$} & $0.866$\tiny{$\pm0.012$} & $0.867$\tiny{$\pm0.008$} & $0.872$\tiny{$\pm0.008$} & $0.860$\tiny{$\pm0.020$} & $0.871$\tiny{$\pm0.006$} \\
Human Enhancer Ensembl  & $0.895$\tiny{$\pm0.002$} & $0.915$\tiny{$\pm0.001$} & $0.920$\tiny{$\pm0.006$} & $0.892$\tiny{$\pm0.004$} & $0.909$\tiny{$\pm0.004$} & $0.915$\tiny{$\pm0.005$} \\
Human Enhancers Cohn    & $0.739$\tiny{$\pm0.007$} & $0.742$\tiny{$\pm0.005$} & $0.741$\tiny{$\pm0.007$} & $0.743$\tiny{$\pm0.007$} & $0.736$\tiny{$\pm0.008$} & $0.738$\tiny{$\pm0.004$} \\
Human vs. Worm          & $0.970$\tiny{$\pm0.002$} & $0.973$\tiny{$\pm0.002$} & $0.974$\tiny{$\pm0.001$} & $0.970$\tiny{$\pm0.002$} & $0.972$\tiny{$\pm0.001$} & $0.971$\tiny{$\pm0.003$} \\
Coding vs. Intergenomic & $0.911$\tiny{$\pm0.001$} & $0.920$\tiny{$\pm0.003$} & $0.923$\tiny{$\pm0.002$} & $0.913$\tiny{$\pm0.002$} & $0.917$\tiny{$\pm0.001$} & $0.921$\tiny{$\pm0.003$} \\
Mouse Enhancers         & $0.708$\tiny{$\pm0.052$} & $0.722$\tiny{$\pm0.046$} & $0.721$\tiny{$\pm0.031$} & $0.688$\tiny{$\pm0.022$} & $0.710$\tiny{$\pm0.009$} & $0.740$\tiny{$\pm0.083$} \\ 
\bottomrule
\end{tabular}
\end{sc}
\end{scriptsize}
\end{table*}

==> tables/genomic_benchmark_ablation_model_modules.tex <==
\begin{table*}[ht!]
\centering
\vspace{-6mm}
\caption{Performance comparison of Mamba-based models on genomic benchmarks. Accuracy values with error bars (±) are reported.}
\vspace{2mm}
\label{tab:module_ablation_on_genomic_benchmarks}
\begin{scriptsize}
\begin{sc}
\begin{tabular}{l@{\hskip 0.2em}c@{\hskip 0.2em}c@{\hskip 0.2em}c@{\hskip 0.2em}c}
\toprule
\textbf{Dataset} & \textbf{Mamba-Attn-FFN-MoE} & \textbf{Mamba-FFN-MoE} & \textbf{Mamba-Attn-FFN} & \textbf{Mamba-FFN} \\ 
\midrule
Human OCR Ensembl       & 0.826±0.003          & \textbf{0.832±0.001} & \underline{0.832±0.002}    & 0.831±0.001          \\
Human NonTATA Promoters & \textbf{0.976±0.004} & 0.973±0.002          & 0.966±0.010          & \underline{0.975±0.002}    \\
Human Regulatory        & 0.866±0.006          & \underline{0.873±0.006}    & 0.866±0.003          & \textbf{0.875±0.004} \\
Human Enhancer Ensembl  & \underline{0.922±0.000}    & \textbf{0.924±0.001} & \textbf{0.924±0.001} & 0.920±0.004          \\
Human Enhancers Cohn    & \textbf{0.746±0.005} & 0.742±0.005          & \underline{0.744±0.007}    & 0.741±0.006          \\
Human vs. Worm          & \textbf{0.974±0.000} & \textbf{0.974±0.000} & 0.974±0.001          & 0.974±0.001          \\
Coding vs. Intergenomic & \textbf{0.922±0.002} & \textbf{0.922±0.002} & 0.919±0.003          & \underline{0.921±0.003}    \\
Mouse Enhancers         & 0.767±0.007          & \textbf{0.779±0.006} & 0.715±0.000          & \underline{0.775±0.023}   \\
\bottomrule
\end{tabular}
\end{sc}
\end{scriptsize}
\end{table*}


